Graph Vulnerability and Robustness: A Survey

The study of network robustness is a critical tool in the characterization and sense making of complex interconnected systems such as infrastructure, communication and social networks. While significant research has been conducted in all of these areas, gaps in the surveying literature still exist. Answers to key questions are currently scattered across multiple scientific fields and numerous papers. In this survey, we distill key findings across numerous domains and provide researchers crucial access to important information by--(1) summarizing and comparing recent and classical graph robustness measures; (2) exploring which robustness measures are most applicable to different categories of networks (e.g., social, infrastructure; (3) reviewing common network attack strategies, and summarizing which attacks are most effective across different network topologies; and (4) extensive discussion on selecting defense techniques to mitigate attacks across a variety of networks. This survey guides researchers and practitioners in navigating the expansive field of network robustness, while summarizing answers to key questions. We conclude by highlighting current research directions and open problems.

==> tables/notation/adjacency.tex <==
\begin{table}
    \begin{tabular}[t]{l l}
    \toprule
    \textbf{Symbol} & \textbf{Adjacency Matrix Definitions} \\
    \midrule
        $\bm{A}$ & adjacency matrix \\
        $\bm{A}_{i,j}$ & element at \textit{i}th row, \textit{j}th col. \\
        $\bm{u}(i)$ & eigenvector at position $i$ \\
        $\rho = \lambda_1$ & spectral radius = 1st eigenvalue \\
        $\lambda_d$ & spectral gap \\
        $\bar{\lambda}$ & natural connectivity \\
        %  $SC(i)$ & Sugraph centrality of node $i$ \\
        $\xi$ & spectral scaling \\
        $r_k$ & generalized robustness index \\
    \bottomrule
    \end{tabular}
    \caption{Symbols and definition table for robustness measures based on adjacency matrix.}
    \label{table:notation-adj}
\end{table}

==> tables/notation/graph.tex <==
\begin{table}[h]
\small
\setlength{\tabcolsep}{14pt}

    \begin{tabular}[t]{l l}
    \toprule
    \textbf{Symbol} & \textbf{Graph Definitions} \\
    \midrule
        $G(\altmathcal{V}$, $\altmathcal{E})$ & graph $G$, set of nodes $\altmathcal{V}$, edges $\altmathcal{E}$ \\
        $n, m$ & number nodes $|V|$, edges $|\altmathcal{E}|$ \\
        $\kappa$, $\kappa_v$, $\kappa_e$ & binary, vertex, edge connectivity \\
        $\bar{d}, d_{max}$ & average distance, diameter \\
        $\bar{b}_v$, $\bar{b}_e$ & average vertex, edge betweenness \\
        $C$ & global clustering coefficient \\
        $L$ & largest connected component \\
    \bottomrule
    \end{tabular}
    \caption{Symbols and definition table for robustness measures based on graph connectivity.}
    \label{table:notation-graph}
\end{table}

==> tables/notation/laplacian.tex <==
\begin{table}
    \begin{tabular}[t]{l l} 
    \toprule
    \textbf{Symbol} & \textbf{Laplacian Matrix Definitions} \\
    \midrule
        $\bm{L}$ & laplacian matrix \\
        $\bm{L}_{i,j}$ & element at \textit{i}th row, \textit{j}th col. \\
        $\bm{D}$ & diagonal matrix \\
        $d_i$ & degree of node $i$ \\
        $\mu_1$ & smallest eigenvalue of $\bm{L}$ \\
        $\mu_2$ & algebraic connectivity of $\bm{L}$ \\
        $T$ & number of spanning trees \\
        $R$ & effective resistance \\
    \bottomrule
    \end{tabular}
    \caption{Symbols and definition table for robustness measures based on Laplacian matrix.}
    \label{table:notation-lap}
\end{table}
